GPTs are GPTs: An Early Look at the Labor Market Impact Potential of Large Language Models

We investigate the potential implications of large language models (LLMs), such as Generative Pre-trained Transformers (GPTs), on the U.S. labor market, focusing on the increased capabilities arising from LLM-powered software compared to LLMs on their own. Using a new rubric, we assess occupations based on their alignment with LLM capabilities, integrating both human expertise and GPT-4 classifications. Our findings reveal that around 80% of the U.S. workforce could have at least 10% of their work tasks affected by the introduction of LLMs, while approximately 19% of workers may see at least 50% of their tasks impacted. We do not make predictions about the development or adoption timeline of such LLMs. The projected effects span all wage levels, with higher-income jobs potentially facing greater exposure to LLM capabilities and LLM-powered software. Significantly, these impacts are not restricted to industries with higher recent productivity growth. Our analysis suggests that, with access to an LLM, about 15% of all worker tasks in the US could be completed significantly faster at the same level of quality. When incorporating software and tooling built on top of LLMs, this share increases to between 47 and 56% of all tasks. This finding implies that LLM-powered software will have a substantial effect on scaling the economic impacts of the underlying models. We conclude that LLMs such as GPTs exhibit traits of general-purpose technologies, indicating that they could have considerable economic, social, and policy implications.

==> ONET_Basic_Skills_Defintions.tex <==


 ONET Basic SKills
 
 Reading Comprehension — Understanding written sentences and paragraphs in
work related documents.
 Active Listening — Giving full attention to what other people are saying, taking
time to understand the points being made, asking questions as appropriate, and not
interrupting at inappropriate times.
 Writing — Communicating effectively in writing as appropriate for the needs of
the audience.
 Speaking — Talking to others to convey information effectively.
 Mathematics — Using mathematics to solve problems.
 Science — Using scientific rules and methods to solve problems.
 Process — Procedures that contribute to the more rapid acquisition of knowledge and
skill across a variety of domains
 Critical Thinking — Using logic and reasoning to identify the strengths and
weaknesses of alternative solutions, conclusions or approaches to problems.
 Active Learning — Understanding the implications of new information for both
current and future problem-solving and decision-making.
 Learning Strategies — Selecting and using training/instructional methods and
procedures appropriate for the situation when learning or teaching new things.
 Monitoring — Monitoring/Assessing performance of yourself, other individuals,
or organizations to make improvements or take corrective action.

==> tables/demographics_table.tex <==
\centering
\begin{tabular}{l r r r r r r}
\toprule
& \multicolumn{1}{l}{\textbf{coef}} & \multicolumn{1}{l}{\textbf{std err}} & \multicolumn{1}{l}{\textbf{z}} & \multicolumn{1}{l} {\textbf{P$> |$z$|$}} & \multicolumn{1}{l}{\textbf{[0.025}} & \multicolumn{1}{r}{\textbf{0.975]}} \\
\midrule
\textbf{const}    &       0.1814  &        0.014     &    12.509  &         0.000        &        0.153    &        0.210     \\
\textbf{women}    &       0.0961  &        0.016     &     6.017  &         0.000        &        0.065    &        0.127     \\
\textbf{black}    &      -0.0794  &        0.066     &    -1.204  &         0.229        &       -0.209    &        0.050     \\
\textbf{asian}    &       0.2231  &        0.083     &     2.674  &         0.008        &        0.060    &        0.387     \\
\textbf{hispanic} &      -0.3934  &        0.040     &    -9.811  &         0.000        &       -0.472    &       -0.315     \\
\bottomrule
\end{tabular}

==> tables/reg_results_other_measures.tex <==

\begin{table}[h]
\centering
\caption{OLS Regression Results of Related AI Exposure Measures on GPT-4 E Labels (Occupation Level)}
\newcolumntype{C}[1]{>{\centering\arraybackslash}p{#1}}
\begin{tabular}{lC{1.5cm}cccccc}
\hline
Variable & Coefficient & Std. Error & P$>|$t$|$ & 95\% CI Lower & 95\% CI Upper \\
\hline
Intercept & -1.1294 & 0.272 & 0.000 & -1.663 & -0.596 \\
Software (Webb) & 0.0011 & 0.000 & 0.000 & 0.001 & 0.002 \\
Robots (Webb) & -0.0038 & 0.000 & 0.000 & -0.004 & -0.003 \\
AI (Webb) & 0.0008 & 0.000 & 0.010 & 0.000 & 0.001 \\
Suitability for ML & 0.2952 & 0.046 & 0.000 & 0.206 & 0.385 \\
Normalized Routine Cognitive & 0.0660 & 0.009 & 0.000 & 0.048 & 0.084 \\
Normalized Routine Manual & -0.1115 & 0.008 & 0.000 & -0.127 & -0.096 \\
AI Exposure (FRS) & 0.0099 & 0.011 & 0.377 & -0.012 & 0.032 \\
Frey and Osborne & -0.0302 & 0.019 & 0.104 & -0.067 & 0.006 \\
Log(Mean Salary) & 0.0580 & 0.019 & 0.002 & 0.021 & 0.095
\end{tabular}

\vspace{1em} % Add some space between the tables
\begin{tabular}{ll}
Dep. Variable: & Mean GPT-4 Exposure Rating \\
Model: & OLS \\
No. Observations: & 680 \\
R-squared: & 0.712 \\
Adj. R-squared: & 0.708 \\
F-statistic: & 222.2 \\
\end{tabular}
\label{tab:validation}
\end{table}
